Seeking Interpretability and Explainability in Binary Activated Neural Networks

We study the use of binary activated neural networks as interpretable and explainable predictors in the context of regression tasks on tabular data; more specifically, we provide guarantees on their expressiveness, present an approach based on the efficient computation of SHAP values for quantifying the relative importance of the features, hidden neurons and even weights. As the model's simplicity is instrumental in achieving interpretability, we propose a greedy algorithm for building compact binary activated networks. This approach doesn't need to fix an architecture for the network in advance: it is built one layer at a time, one neuron at a time, leading to predictors that aren't needlessly complex for a given task.

==> sections/sparse.tex <==
The sparseness of the predictors the BGN yields has been discussed in the paper, but not empirically supported. Two experiments have been conducted in order to demonstrate it. On two different datasets, networks with hidden layers of width respectively 100-100-20 and 100-65 have been built. \autoref{fig:sparse_1} and \autoref{fig:sparse_2} clearly show that the BGN predictors are composed of many 0-valued parameters, meaning that only the relevant parameters are non-zeros. Also, those two figures highlight the fact that BGN predictors are consistent; their number of parameters are quite stable.

\begin{figure}
\begin{center}
\includegraphics[width=0.6\linewidth]{figures/sparseness_carbon.png} \caption{Mean and standard deviation over three repetitions of the number of non-zero parameters of the predictor yeilded by BGN over it's training on the Carbon nanotubes dataset versus the maximum number of parameter a NN with a similar architecture could have.}\label{fig:sparse_1}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.6\linewidth]{figures/sparseness_hung_pox.png} \caption{Mean and standard deviation over three repetitions of the number of non-zero parameters of the predictor yeilded by BGN over it's training on the Hungarian chickenpox cases dataset versus the maximum number of parameter a NN with a similar architecture could have.}\label{fig:sparse_2}
\end{center}
\end{figure}

